Seed1.5-Thinking: Advancing Superb Reasoning Models with Reinforcement Learning

We introduce Seed1.5-Thinking, capable of reasoning through thinking before responding, resulting in improved performance on a wide range of benchmarks. Seed1.5-Thinking achieves 86.7 on AIME 2024, 55.0 on Codeforces and 77.3 on GPQA, demonstrating excellent reasoning abilities in STEM and coding. Beyond reasoning tasks, the method demonstrates notable generalization across diverse domains. For instance, it surpasses DeepSeek R1 by 8% in win rate on non-reasoning tasks, indicating its broader applicability. Compared to other state-of-the-art reasoning models, Seed1.5-Thinking is a Mixture-of-Experts (MoE) model with a relatively small size, featuring 20B activated and 200B total parameters. As part of our effort to assess generalized reasoning, we develop two internal benchmarks, BeyondAIME and Codeforces, both of which will be publicly released to support future research. Model trial link: https://www.volcengine.com/experience/ark.

==> sections/110contributions.tex <==
\newpage
\twocolumn
\section*{Contributions and Acknowledgments}


\subsection*{\textcolor{brown}{Core Contributors}}
(Author names randomly shuffled) \\
Yufeng Yuan \\
Yu Yue \\
Mingxuan Wang \\
Xiaochen Zuo \\ 
Jiaze Chen \\
Lin Yan \\
Wenyuan Xu \\
Chi Zhang \\
Xin Liu \\
Chengyi Wang \\
TianTian Fan \\
Lingjun Liu \\
Qiying Yu \\
Xiangpeng Wei \\
Zhiqi Lin \\

\subsection*{Contributors}
Ruofei Zhu \\
Qingping Yang \\
Chengzhi Wei \\
Jerry He \\
Guanlin Liu \\
Zheng Wu* \footnote{* represents members who have departed from the team} \\
Renjie Zheng \\
Xiangyu Yu \\
Zhicheng Liu \\
Jingjing Xu \\
Jiangjie Chen \\
Haojie Pan \\
Shengding Hu* \\
Zhengyin Du \\
Wenqi Wang \\
Zewei Sun \\
Chenwei Lou \\
Shuangzhi Wu \\
Hang Zhu \\
Bole Ma \\
Zihan Wang \\
Mofan Zhang \\
Wang Zhang \\
Gaohong Liu \\
Kaihua Jiang \\
Haibin Lin \\
Ru Zhang \\
Juncai Liu \\
Li Han \\
Jinxin Chi \\
Meng Qu \\
Wei Shen \\

\subsection*{Pretraining Efforts}
Wenqiang Zhang\\
Jiayi Xu \\
Jun Yuan \\
Zhen Xiao \\
Yuqiao Xian \\
Jingqiao Wu \\
Kai Hua \\
Na Zhou \\
Jianhui Duan \\
Heyang Lu \\
Changbao Wang \\
Jinxiang Ou \\
Shihang Wang \\
Xiaoran Jin \\
Xuesong Yao \\
Chengyin Xu \\
Wenchang Ma \\
Zhecheng An \\
Renming Pang \\
Xia Xiao \\
Jing Su \\
Yuyu Zhang \\
Tao Sun \\
Kaibo Liu \\
Yifan Sun \\
Kai Shen \\
Sijun Zhang \\
Yiyuan Ma \\
Xingyan Bin \\
Ya Wang \\
Yao Luo \\
Deyi Liu \\
Shiyi Zhan \\
Yunshui Li \\
Yuan Yang \\
Defa Zhu \\
Ke Shen \\
Chenggang Li \\
Xun Zhou \\
Liang Xiang \\

\subsection*{Team Lead}

Yonghui Wu \\

\onecolumn

==> sections/120contributions.tex <==
\newpage
\section*{Contributions and Acknowledgments}
(Author names randomly shuffled)\\
Yufeng Yuan,
Yu Yue,
Mingxuan Wang,
Xiaochen Zuo,
Jiaze Chen,
Lin Yan,
Wenyuan Xu,
Chi Zhang,
Xin Liu,
Chengyi Wang,
TianTian Fan,
Lingjun Liu,
Qiying Yu,
Xiangpeng Wei,
Zhiqi Lin,

\subsection*{\textcolor{brown}{Core Contributors}}
(Author names randomly shuffled) \\
Yufeng Yuan, 
Yu Yue, 
Mingxuan Wang, 
Xiaochen Zuo,  
Jiaze Chen, 
Lin Yan, 
Wenyuan Xu, 
Chi Zhang, 
Xin Liu, 
Chengyi Wang, 
TianTian Fan, 
Lingjun Liu, 
Qiying Yu, 
Xiangpeng Wei, 
Zhiqi Lin
Yonghui Wu

\subsection*{Contributors}
Ruofei Zhu, 
Qingping Yang, 
Chengzhi Wei, 
Jerry He, 
Guanlin Liu, 
Zheng Wu* \footnote{* represents members who have departed from the team}, 
Renjie Zheng, 
Xiangyu Yu, 
Zhicheng Liu, 
Jingjing Xu, 
Jiangjie Chen, 
Haojie Pan, 
Shengding Hu*, 
Zhengyin Du, 
Wenqi Wang, 
Zewei Sun, 
Chenwei Lou, 
Shuangzhi Wu, 
Hang Zhu, 
Bole Ma, 
Zihan Wang, 
Mofan Zhang, 
Wang Zhang, 
Gaohong Liu, 
Kaihua Jiang, 
Haibin Lin, 
Ru Zhang, 
Juncai Liu, 
Li Han, 
Jinxin Chi, 
Meng Qu, 
Wei Shen

\subsection*{Pretraining Efforts}
Wenqiang Zhang, 
Jiayi Xu, 
Jun Yuan, 
Zhen Xiao, 
Yuqiao Xian, 
Jingqiao Wu, 
Kai Hua, 
Na Zhou, 
Jianhui Duan, 
Heyang Lu, 
Changbao Wang, 
Jinxiang Ou, 
Shihang Wang, 
Xiaoran Jin, 
Xuesong Yao, 
Chengyin Xu, 
Wenchang Ma, 
Zhecheng An, 
Renming Pang, 
Xia Xiao, 
Jing Su, 
Yuyu Zhang, 
Tao Sun, 
Kaibo Liu, 
Yifan Sun, 
Kai Shen, 
Sijun Zhang, 
Yiyuan Ma, 
Xingyan Bin, 
Ya Wang, 
Yao Luo, 
Deyi Liu, 
Shiyi Zhan, 
Yunshui Li, 
Yuan Yang, 
Defa Zhu, 
Ke Shen, 
Chenggang Li, 
Xun Zhou, 
Liang Xiang

\subsection*{Team Lead}

Yonghui Wu

